Synthetic dataset of ID and Travel Document

This paper presents a new synthetic dataset of ID and travel documents, called SIDTD. The SIDTD dataset is created to help training and evaluating forged ID documents detection systems. Such a dataset has become a necessity as ID documents contain personal information and a public dataset of real documents can not be released. Moreover, forged documents are scarce, compared to legit ones, and the way they are generated varies from one fraudster to another resulting in a class of high intra-variability. In this paper we trained state-of-the-art models on this dataset and we compare them to the performance achieved in larger, but private, datasets. The creation of this dataset will help to document image analysis community to progress in the task of ID document verification.

==> technical_validation.tex <==
\section*{Technical Validation}
%This section presents any experiments or analyses that are needed to support the technical quality of the dataset. This section may be supported by figures and tables, as needed. This is a required section; authors must present information justifying the reliability of their data.


Data is partitioned to allow three model validation techniques: {\bf hold-out},  {\bf k-fold cross-validation} and {\bf few-shot}. The code provided allow users to define any partition for these three  model validation schemes. Data is randomly sampled and it is, by default, split into 80\%-10\%-10\% for the hold-out validation and split it into 10 folds for the k-fold cross-validation. For few-shot, 6 nationalities ID documents are randomly chosen for the meta-training and the remainder 4 for the meta-testing. However, for fair comparison between models we also provide a predefined partition in which training, validation and test instances are always the same for both, the hold-out and the k-fold cross-validation.


%Regarding the \textit{hold-out} partition, the data is randomly split into 80\% - 10\% - 10\% partitions.  Whereas in the \textit{K-fold cross-validation}, our models are trained according to 10-fold cross validation, eight folds for training, one fold for validation, and one for test set.



%Two different data partitions are set up in order to train, validate, and test the performance of our set of models: {\bf hold-out} \& {\bf k-fold cross validation}.
%Regarding the \textit{hold-out} partition, the data is randomly split into 80\% - 10\% - 10\% partitions.  Whereas in the \textit{K-fold cross-validation}, our models are trained according to 10-fold cross validation, eight folds for training, one fold for validation, and one for test set.

%To enable the replication of the diverse results, each partition set up is recorded in a file in a static way.
%for each partition set up, we have established a file with a static partition. 
%The file contains the file paths of the documents from the dataset utilized in generating the results. 
%\textcolor{red}{The partitions were created based on the documents, regardless of the number of instances in which a given document appears. 
%This ensures that both counterfeit clips and videos were produced by sampling counterfeit templates.
%This approach was chosen to uphold dataset consistency.} \textbf{Not clear}

%\\
%To enable the replication of diverse results, we have established distinct files with static partitions. Each file contains the file paths of the documents utilized in generating the results. Consequently, four partitions have been defined: two for the templates, ensuring balance, and two for the videos and clips, characterized by an imbalance. The imbalance observed in the clips and videos partition is attributed to the time-intensive nature of video generation. However, this imbalance effectively emulates real-world scenarios where counterfeit IDs are exceedingly rare

To evaluate the SIDTD dataset, we have trained five state-of-the-art deep learning models for three tasks: {\bf template-based ID documents},  {\bf video-based ID documents} and {\bf Few-shot}. The template-based ID documents tasks evaluate the performance of the selected models to detect forged document that have solely altered by  {\em Composite} PAIs. The video-based ID document task evaluate the performance of the same models when the images comes from a video recording. The few-shot task is a quite more realistic task as models are trained for a given subset of nationalities and test on ID documents from other nationalities. Finally, to compare the dataset difficulty we compare the performance of the benchmark models on a private, and not available, dataset.



%balanced classification and unbalanced classification. The classification tasks use all templates with their corresponding labels from the SIDTD dataset. So as to compare  models performance on this dataset, we have also trained the models on a private (and larger) dataset and test them using a dataset that contains real forged ID documents from IDN. It is worth noting that the images for this real dataset are pictures from {\em bona fide} or forged documents with capturing conditions and backgrounds different from those fril the balanced SIDTD used in the models training. %However, for this dataset the images are pictures from {\em bona fide} or forged documents with background unlike the training performed on the balanced SIDTD that was performed on identity document templates.




\subsection*{Deep Learning models}


The following five models were used to evaluate the SIDTD dataset: EfficientNet-B3~\cite{tan2019efficientnet}, ResNet50~\cite{he2016deep}, Vision Transformer Large Patch 16 (ViT-L/16)~\cite{dosovitskiy2020vit}, TransFG~\cite{he2022transfg} and Co-Attention Attentive Recurrent Network (CoAARC)~\cite{Berenguel:2019,wu2020acr}. 
EfficientNet, ResNet, and ViT models are general purpose models while TransFG is a model for fine-grained classification task while the CoAARC  model was designed to detect forged ID documents.

The EfficientNet-B3 and  ResNet-50 models are convolutional models widely used by the deep learning community for general purpose classification tasks. EfficientNet is a network model designed to use its  parameters more efficiently, optimising both accuracy and FLOPS\footnote{FLOPS = Floating point operations per second}, which has resulted in models with fewer parameters but equally accurate. ViT-L/16 and TransFG are models inspired by the Transformer\cite{vaswani2017attention} encoder architecture from NLP models. The Vision Transformer (ViT) model links each patch to the classification token through a self-attention mechanism based on a Transformer encoder. The TransFG models is an extension of the ViT model. Its main innovation is the addition of a Part Selection Module that selects the tokens that bring valuable information in order to use only discriminative image patches. We use the same type of ViT model for TransFG as a base network: ViT-L/16. %TransFG is adapted from the code of \cite{he2022transfg}'s paper. %
The CoAARC model  is an algorithmic imitation of the human way that compares alternatively two images. The model contains a co-attention mechanism that focuses on identifying the most relevant and crucial parts of the images. For the given PAD task it focus on learning the differences between {\em bona fide} and forged ID Documents.

The EfficientNet-B3, ResNet50 and ViT-L/16 are built-in models from PyTorch\footnote{PyTorch site: https://pytorch.org} packages. ViT and CoAARC are trained with an input image resolution of $224x224x3$, and EfficientNet-B3, ResNet50 and TransFG with image resolution of 299x299x3. Each model is pretrained on the ImageNet\cite{deng2009imagenet} dataset. %Trained models are available at the CVC repository.

\subsection*{Private Dataset}

To compare the  SIDTD dataset  to real, but private, industry datasets, we evaluate the performance of the above-mentioned models on a industry dataset composed of real-life images from the \emph{IDNow}\footnote{https://www.idnow.io/} production flow. These images are captured using various devices (scan, smartphone) without any constraint.  As in a real-world dataset there are much less forged ID documents than {\em bona fide} ones, the sub-set of forged ID documents is mainly created by the following {\em Composite} PAI techniques: % generating several examples using:
\begin{itemize}
    \item \textbf{Copy \& Paste} operations inside the same document. Similar to the {\em Crop \& Replace} technique described above, the personal data fields from a real document are firstly located. Then, a source and a target fields are randomly selected and the content of the source field is copied and pasted in the target field.
    \item \textbf{Copy \& Move} operations. Similar to the {\em Crop \& Replace} technique described above, a forged document  is created from a real document by replacing its original identity photo with another one randomly selected from a given set of identity photos. 
\end{itemize}

The data set of this private dataset is finally composed of $1,000$ {\em bona fide} examples and their corresponding $1,000$ {\em forged} examples. All the documents of this data set, whether {\em bona fide} or forged, are of various types (identity car, passports, driving licence, resident permit, etc.) from different countries (France, Spain, Italy, Romania, etc.). 


%belonging to the following PAI types.
%\begin{itemize}
 %   \item Fully generated: the document images of this type are generated from scratch using a predefined template identical to a real one. This template is filled with personal data to create an improper identity document.    
    %\item Composition: this type of fraud consist on changing the personal data (photo, first names, last names, dates, etc.)  within a document image using various image editing tools.
  %  \item Composition: this type of fraud consist on changing the personal data (photo, first names, last names, dates, etc.)  within a {\em bona fide} document image using copy-paste tool. The position and content can be changed, but the text font remains the same as in a {\em bona fide} document.
   % \item Screen: these documents are captured form  existing images that are displayed in screens and do not necessarily correspond to real identity documents (and if so, they may not belong to the persons capturing them)  
%    \item Printed: these documents are captured from an existing paper copy of an identity documents and not from its original version. As a PAI, it is similar to that containing images captured from screen.   
 %   \item Truncated: this subset contains documents that are cut by the issuing authority to invalidate them. 
%\end{itemize}

%All the documents of this data set, whether {\em bona fide} or forged, are of various types (identity car, passports, driving licence, resident permit, etc.) from different countries (France, Spain, Italy, Romania, etc.). 

%The Table \ref{tab:AXT_private_dataset} shows some statistics on this data set. 

%\begin{table}[h]
%\centering
%\begin{tabular}{|l|l|l|}
%\hline
%\multicolumn{1}{|c|}{\textbf{Class}} & \multicolumn{1}{c|}{\textbf{PAI}} & \multicolumn{1}{c|}{\textbf{Number of samples}} \\ \hline
%{\em bona fide}                 & N/A               & 10.397     \\ \hline
%\multirow{5}{*}{Forged}               & Fully generated   & 3.200      \\ \cline{2-3} 
 %                               & Composition       & 1.669      \\ \cline{2-3} 
  %                              & Screen            & 2.336      \\ \cline{2-3} 
   %                             & Printed           & 2.000      \\ \cline{2-3} 
    %                            & Truncated           & 2.017      \\ \hline
%\end{tabular}
%\caption{Private data set extracted from IDNow production flow.}
%\label{tab:AXT_private_dataset}
%\end{table}



\subsection*{Results}

Most of the models performs well in the two supervised tasks on the SIDTD and private dataset. The challenge of verifying if an ID or travel document image comes from an original document or it has been modified, or forged, by any means is relatively easy if models are trained with enough data from a given set of the nationalities. The problem comes when models try to verify whether ID or travel documents of unknown nationalities have been forged or not. The results for the Few-shot task support this thesis. Models performance drop down for all them in both metrics: accuracy and ROC AUC. The same behavior is observed on the private datasets. Model performance are overall good but performance drops on a few-shot scenario.

%We obtained outstanding results on both datasets with most of the models. 

%Models based on convolutional networks (EfficientNet and ResNet) achieved similar  and almost flawless results regardless the type of instances (templates or clips) and datasets (SIDTD and Private). Same conclusion could be drawn from the recurrent network (CoAARN). However,  The Vision Transformer-based models improved radically the performance on clips cropped SIDTD. One hypothesis that could explain that variation is the dataset size and diversity that could benefit to larger models. \colorbox{red}{ViT performance is poor on the balanced dataset, shouldn't we explain why?}


\begin{table}[h]
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{|c|c|c|c|c|c|c|c|c|} 
\hline
 \multirow{2}{*}{Dataset} &  \multicolumn{2}{c|}{Templates-based task }  & \multicolumn{2}{c|}{Video-based task}  &   \multicolumn{2}{c|}{ Few-shot  task} & \multicolumn{2}{c|}{Private dataset }  \\   \cline{2-9} 
  & accuracy & ROC AUC & accuracy & ROC AUC & accuracy & ROC AUC & accuracy & ROC AUC \\
\hline 
EfficientNet & $0.994 \pm 0.010$ & $1.000 \pm 0.000$ & $0.999 \pm 0.001$ & $1.000 \pm 0.000$   &  $0.593 \pm 0.023$ & $0.623 \pm 0.036$ & $0.987 \pm 0.000$ & $0.998 \pm 0.000$ \\  %\hline 
ResNet & $0.981 \pm 0.012$ & $1.000 \pm 0.011$ & $0.999 \pm 0.002$ & $1.000 \pm 0.000$  &  $0.635 \pm 0.058$ & $0.669 \pm 0.073$ & $0.984 \pm 0.000$ & $0.996 \pm 0.000$ \\ 
\hline 
ViT & $0.552 \pm 0.023$ & $0.501 \pm 0.042$ & $0.975 \pm 0.020$ & $0.989 \pm 0.015$ &  $0.609 \pm 0.026$ & $0.645 \pm 0.032$ & $0.792 \pm 0.023$ & $0.872 \pm 0.000$  \\  %\hline 
TransFG & $0.966 \pm 0.015$ & $0.992 \pm 0.004$ & $0.999 \pm 0.002$  & $1.000 \pm 0.000$ & $0.582 \pm 0.038$ & $0.612 \pm 0.049$ &  $- \pm -$ & $- \pm -$ \\ 
\hline 
CoAARN & $0.986 \pm 0.016$ & $0.999 \pm 0.003$ & $0.992 \pm 0.012$ & $0.999 \pm 0.003$ &  $0.530 \pm 0.020$ & $0.539  \pm 0.027$ &  $- \pm -$ & $- \pm -$ \\ 
\hline 
\end{tabular} 
}
\caption{Models performance in  terms of accuracy and ROC AUC  scores with standard deviation. Models are trained and test regarding a 10-fold cross-validation for the template-based ID document and the Video-based ID document tasks. Model performance is also reported for the Private dataset from IDNow. }
\label{tab:all_results}
\end{table}


% \subsection*{Private dataset Results}

% \begin{table}[h]
% \centering
% \begin{tabular}{|c|c|c|c|c|} 
% \hline
%  Dataset &  \multicolumn{2}{c|}{IDnow_{tr}}  & \multicolumn{2}{c|}{IDnow_{te}}  \\ 
% \hline 
%  Metrics & accuracy & ROC AUC & accuracy & ROC AUC \\
% \hline 
% EfficientNet & $0.987 \pm 0.000$ & $0.998 \pm 0.000$ &  &  \\  %\hline 
% ResNet & $0.984 \pm 0.000$ & $0.996 \pm 0.000$ & & \\ 
% \hline 
% ViT & $0.792 \pm 0.023$ & $0.872 \pm 0.000$ &  & \\  %\hline 
% TransFG & &  & &  \\ 
% \hline 
% CoAARN & & & & \\ 
% \hline 
% \end{tabular} 
% \caption{Models' results are shown in terms of ROC AUC and accuracy scores with standard deviation. Models are trained and test regarding a 10-fold cross validation.  IDnow$_{tr}$ is a balanced dataset and contains picture with background from real-world forged and real identity documents. IDnow$_{te}$ is an unbalanced dataset and contains picture with background from real-world real identity documents and different forgery than IDnow$_{tr}$.}
% \label{tab:all_results}
% \end{table}



%\subsection*{Training set up}

%At each batch we equally draw documents from Templates and clips cropped SIDTD with a uniform probability in order to have a balanced batch between both type of documents.

%We added a specific data augmentation designed to enhance models performance by generating new forged documents on-the-fly which is meant to reduce the likelihood of model overfitting. 75\% of the batch size is composed of {\em bona fide} documents and 25\% of forged documents. Then, during the training, we extract one third of the {\em bona fide} documents in order to generate new fake documents. Hence, we end up with a batch of documents composed of 50\% of {\em bona fide} documents and 50\% of forged documents (to image how we generate batch, see \figurename~\ref{fig:batchorga} with batch size of 32 as an exemple)

%\begin{figure}[h]
%\begin{center}
% \includegraphics[width=0.85\columnwidth]{mixedmidv2020_forgeryonthefly.png}
%\end{center}
%\caption{Scheme of batch generation with a batch size of 32 to illustrate.}\label{fig:batchorga}
%\end{figure}


%Data are preprocessed regarding the following procedure: resizing, normalization and data augmentation. We trained our network on distinct types of GPUs: NVIDIA A40, Quadro RTX 6000 and NVIDIA GeForce RTX 3090.


%The average accuracy and Area Under de Curve (AUC) for all the tasks are shown in Tables~\ref{tab:results_accuracy} and \ref{tab:results_roc_auc}.





%\subsection*{Statistical evaluation}
%%TODO 
%We must perform statistical analysis to validate (hopefully) correlation on the AUC scores and/or Accuracies scores between SIDTD  and private datasets


